PhilHumans: Benchmarking Machine Learning for Personal Health

The use of machine learning in Healthcare has the potential to improve patient outcomes as well as broaden the reach and affordability of Healthcare. The history of other application areas indicates that strong benchmarks are essential for the development of intelligent systems. We present Personal Health Interfaces Leveraging HUman-MAchine Natural interactions (PhilHumans), a holistic suite of benchmarks for machine learning across different Healthcare settings - talk therapy, diet coaching, emergency care, intensive care, obstetric sonography - as well as different learning settings, such as action anticipation, timeseries modeling, insight mining, language modeling, computer vision, reinforcement learning and program synthesis

==> archive_texts.tex <==
Some targeted scenarios of example are listed below.
\begin{itemize}
\item \textit{Emily’s baby Gary has been sleeping very badly in the last few weeks which makes the whole family tired and irritated. Emily turns to the PH health assistant in the kitchen speaker to discuss the problem. It turns out in the discussion that the irregular evening routines may be a cause of Gary’s sleep difficulties. The observation is also verified based on the tracking data which shows that especially in weekends the bedtime of Gary is often very different from weekdays. The PH assistant then engages Emily into a motivating conversation where Emily supported by the assistant finds a way to stabilize the weekend evening routines for Gary. In the next three weeks, Emily and assistant have brief morning discussions about the progress.}   
\item \textit{John is a busy and obese middle-aged engineer who smokes, eats unhealthy, and usually drives his car even short distances. After the first cardiac event, a friend convinces him to get a health watch and install PH health assistant to his car entertainment system. During commute, he now regularly has friendly motivating discussions about his health behavior, inner feelings, and life in general. John has already realized that he can become more active and fresh in the morning at work if he parks the car further away from the work, and take a brisk walk in on the way there and back- it gives 3000 steps!. The assistant in the car also supports John in quitting smoking, and John is even considering to buy a bicycle, something that he has not done in ages.}
\item \textit{Mike has been on drugs for many years. Mike has decided to quit it and rebuild the relation to his children and ex-wife who moved out already a few years ago. In weakest moments he often has short conversations with PH assistant. The assistant mostly listens and reflects what he has said, but this already makes him remember what is most important, that he becomes again a good father and model for his two sons.}
\end{itemize}




\section{Conversational interfaces for health services}

\subsection{Trends in spoken dialog systems and conversation modeling}

\subsection{Trends in automatic content generation}

\subsection{Trends in situational intelligence, context sensing}

\subsection{Trends in First Person (Egocentric) Vision}
Visual perception is the primary means by which humans sense and understand the world. Since vision is a form of intelligence itself, we should expect that building truly intelligent systems which are likely to characterize our personal needs will require the development of advanced forms of AI. While the sensing technologies needed to obtain a suitable visual representation of the world are already available and ready to use, much work is still to be done to enable the design and development of AI algorithms to be embedded in intelligent systems capable of making a real difference in our lives. A promise in this context can be intelligent systems that can be worn by the users to sense the world from their unique point of view. These systems could directly advice the user as well as transfer inferred information to other active systems (e.g., robots) which interact with the user during daily activities with the final aim of assisting the users. To build this kind of personalized systems able to naturally interact with users, First Person (Egocentric) Vision paradigm has an important role~\cite{Kanade2012}. The term First Person Vision (FPV) is generally used to refer to systems which exploit Computer Vision and Machine Learning algorithms to understand images and videos acquired by means of a camera worn by the user. One of the main differences between a wearable camera and a standard fixed one is the intrinsic mobility of the former. The content acquired from FPV cameras always ``tells somethin'' about the behavior of the user, the location in which he is operating, the activities he is involved in and, ultimately, his true intent and goals. Computer Vision and Machine Learning algorithms in this scenario have to face the challenging task to infer information about the user. Despite this kind of wearable computing has long history~\cite{Betancourt2015,Mann97}, it has become of more interest in the last years with the advancement of both hardware and software technologies~\cite{Furnari2017a}. The main applications of FPV systems in the context of assistive Computer Vision~\cite{Leo2017} is related to memory augmentation~\cite{Damen2015} and life logging~\cite{Furnari2018b,Gurrin2014,Ortis2017}. Recent studies have also considered the FPV paradigm to recognize important objects observed by user~\cite{Lee2015} and to understand or to anticipate the actions and activities performed by the user~\cite{Damen2018EPIC,Furnari2018a,Ryoo2016,Singh2016} or the next object to which the user is going to interact with~\cite{Furnari2017c}. Nowadays, the market proposes different FPV devices which can be employed for a variety of purposes (e.g., Google Glass~\footnote{Google Glass, http://www.x.company/glass/}, Microsoft Hololens~\footnote{Microsoft Hololens: https://www.microsoft.com/en-us/hololens}, Magic Leap~\footnote{Magic Leap: https://www.magicleap.com/}, GoPro~\footnote{GoPro: https://gopro.com/}, OrCam~\footnote{OrCam: https://www.orcam.com/}, etc.). Since the cameras is worn by the user and carried with him at all times, FPV data is highly personal~\cite{Lee2015}, and always relevant to understand the user and the performed activities. This property allows the creation of personalized algorithms which can learn from user-specific data providing specialized assistance.

\subsection{Trends in interface devices, robotics, IoT}



==> contributions.tex <==
\chapter{List of contributions}

Let's make a shortlist of philhumans scientific contributions so that we can see what the unifying themes are. We can start by pasting the abstracts of our papers.

\section{Predicting the Future from First Person (Egocentric) Vision: A Survey}

Egocentric videos can bring a lot of information about how humans perceive the world and interact with the environment, which
can be beneficial for the analysis of human behaviour. The research in egocentric video analysis is developing rapidly thanks to the
increasing availability of wearable devices and the opportunities offered by new large-scale egocentric datasets. As computer vision
techniques continue to develop at an increasing pace, the tasks related to the prediction of future are starting to evolve from the need
of understanding the present. Predicting future human activities, trajectories and interactions with objects is crucial in applications
such as human-robot interaction, assistive wearable technologies for both industrial and daily living scenarios, entertainment and
virtual or augmented reality. This survey summarises the evolution of studies in the context of future prediction from egocentric
vision making an overview of applications, devices, existing problems, commonly used datasets, models and input modalities. Our
analysis highlights that methods for future prediction from egocentric vision can have a significant impact in a range of applications
and that further research efforts should be devoted to the standardisation of tasks and the proposal of datasets considering real-world
scenarios such as the ones with an industrial vocation.

\section{Untrimmed Action Anticipation}

Egocentric action anticipation consists in predicting a future action the camera wearer will perform from egocentric video. While
the task has recently attracted the attention of the research community, current approaches assume that the input videos are “trimmed”,
meaning that a short video sequence is sampled a fixed time before the beginning of the action. We argue that, despite the recent advances in the field, trimmed action anticipation has a limited applicability in realworld scenarios where it is important to deal with “untrimmed” video inputs and it cannot be assumed that the exact moment in which the action will begin is known at test time. To overcome such limitations, we propose an untrimmed action anticipation task, which, similarly to temporal action detection, assumes that the input video is untrimmed at test time, while still requiring predictions to be made before the actions actually take place. We design an evaluation procedure for methods designed to address this novel task, and compare several baselines on the EPIC-KITCHENS-100 dataset. Experiments show that the performance of current models designed for trimmed action anticipation is very limited and more research on this task is required.

\section{Scene Understanding and Interaction Anticipation from First Person Vision}

Egocentric videos can bring a lot of information about actions performed by humans, which can be beneficial for the analysis of human activity by an external agent such as a robot. This external agent is used as a personal assistant, it should be able to anticipate the user’s moves, actions and intentions. Action anticipation from first-person cameras is a challenging task due to the nature of the data processed and the non-scripted, as well as person-specific character of actions. This position paper briefly reviews the current state-of-the-art approaches for action anticipation from egocentric video and proposes ideas on how to improve the quality of predictions.

\section{Creation, Analysis and Evaluation of AnnoMI, a Dataset of Expert-Annotated Counselling Dialogues}

Research on the analysis of counselling conversations through natural language processing methods has seen remarkable growth in recent years. However, the potential of this field is still greatly limited by the lack of access to publicly available therapy dialogues, especially those with expert annotations, but it has been alleviated thanks to the recent release of AnnoMI, the first publicly and freely available conversation dataset of 133 faithfully transcribed and expert-annotated demonstrations of high- and low-quality motivational interviewing (MI)—an effective therapy strategy that evokes client motivation for positive change. In this work, we introduce new expert-annotated utterance attributes to AnnoMI and describe the entire data collection process in more detail, including dialogue source selection, transcription, annotation, and post-processing. Based on the expert annotations on key MI aspects, we carry out thorough analyses of AnnoMI with respect to counselling-related properties on the utterance, conversation, and corpus levels. Furthermore, we introduce utterance-level prediction tasks with potential real-world impacts and build baseline models. Finally, we examine the performance of the models on dialogues of different topics and probe the generalisability of the models to unseen topics.

\section{Fully-Unsupervised Embeddings-Based Hypernym Discovery}

The hypernymy relation is the one occurring between an instance term and its general term (e.g., “lion” and “animal”, “Italy” and “country”). This paper we addresses Hypernym Discovery, the NLP task that aims at finding valid hypernyms from words in a given text, proposing HyperRank, an unsupervised approach that therefore does not require manually-labeled training sets as most approaches in the literature. The proposed algorithm exploits the cosine distance of points in the vector space of word embeddings, as already proposed by previous state of the art approaches, but the ranking is then corrected by also weighting word frequencies and the absolute level of similarity, which is expected to be similar when measuring co-hyponyms and their common hypernym. This brings us two major advantages over other approaches—(1) we correct the inadequacy of semantic similarity which is known to cause a significant performance drop and (2) we take into accounts multiple words if provided, allowing to find common hypernyms for a set of co-hyponyms—a task ignored in other systems but very useful when coupled with set expansion (that finds co-hyponyms automatically). We then evaluate HyperRank against the SemEval 2018 Hypernym Discovery task and show that, regardless of the language or domain, our algorithm significantly outperforms all the existing unsupervised algorithms and some supervised ones as well. We also evaluate the algorithm on a new dataset to measure the improvements when finding hypernyms for sets of words instead of singletons.

\section{Creation, Analysis and Evaluation of AnnoMI, a Dataset of Expert-Annotated Counselling Dialogues}

Research on the analysis of counselling conversations through natural language processing methods has seen remarkable growth in recent years. However, the potential of this field is still greatly limited by the lack of access to publicly available therapy dialogues, especially those with expert annotations, but it has been alleviated thanks to the recent release of AnnoMI, the first publicly and freely available conversation dataset of 133 faithfully transcribed and expert-annotated demonstrations of high- and low-quality motivational interviewing (MI)—an effective therapy strategy that evokes client motivation for positive change. In this work, we introduce new expert-annotated utterance attributes to AnnoMI and describe the entire data collection process in more detail, including dialogue source selection, transcription, annotation, and post-processing. Based on the expert annotations on key MI aspects, we carry out thorough analyses of AnnoMI with respect to counselling-related properties on the utterance, conversation, and corpus levels. Furthermore, we introduce utterance-level prediction tasks with potential real-world impacts and build baseline models. Finally, we examine the performance of the models on dialogues of different topics and probe the generalisability of the models to unseen topics.

\section{Unaddressed challenges in persuasive dieting chatbots}

Diet coaching is a behaviour change task which requires lots of interaction with patients. E-health apps gathered lots of interest in research and, recently, chatbots have been leveraged to address this task, with a focus on persuasion to motivate people towards behaviour change. In this paper, we take a look at current approaches in building persuasive dieting chatbots and expose a number of major unsolved challenges. We motivate them with evidence from previous work and show that current chatbots don’t approach certain scenarios properly, hence limiting their communication and persuasion capabilities.

\section{How are you? Introducing stress-based text tailoring}

Can stress affect not only your life but also how you read and interpret a text? Healthcare has shown evidence of such dynamics and in this short paper we discuss customising texts based on user stress level, as it could represent a critical factor when it comes to user engagement and behavioural change. We first show a real-world example in which user behaviour is influenced by stress, then, after discussing which tools can be employed to assess and measure it, we propose an initial method for tailoring the document by exploiting complexity reduction and affect enforcement. The result is a short and encouraging text which requires less commitment to be read and understood. We believe this work in progress can raise some interesting questions on a topic that is often overlooked in NLG.

\section{A NLG Framework for User Tailoring and Profiling in Healthcare}

Communication in healthcare can improve therapy adherence and patient engagement. Research into healthcare-oriented Natural Language Generation (NLG) systems suggests that tailoring to user profile can improve overall effectiveness. However lots of systems adopts a single or small group of user profiles, thus overlooking that user subsets may have different needs and that these could evolve over time. In this paper we conceptualize a framework that can produce cus- tomised healthcare reports by extracting meaningful data insights and producing a final text which varies in content and terminology accord- ing to the user profile and traits. The dietary domain will be used to show a working example.

\section{Beyond calories: evaluating how tailored communication reduces emotional load in diet-coaching}

Dieting is a behaviour change task that is difficult for many people to conduct successfully. This is due to many factors, including stress and cost. Mobile applications offer an alternative to traditional coaching. However, previous work on apps evaluation only focused on dietary outcomes, ignoring users’ emotional state despite its influence on eating habits. In this work, we introduce a novel evaluation of the effects that tailored communication can have on the emotional load of dieting. We implement this by augmenting a traditional diet-app with affective NLG, text-tailoring and persuasive communication techniques. We then run a short 2-weeks experiment and check dietary outcomes, user feedback of produced text and, most importantly, its impact on emotional state, through PANAS questionnaire. Results show that tailored communication significantly improved users’ emotional state, compared to an app-only control group.

\section{Comparing informativeness of an NLG chatbot vs graphical app in diet-information domain}

Visual representation of data like charts and tables can be challenging to understand for readers. Previous work showed that combining visualisations with text can improve the communication of insights in static contexts, but little is known about interactive ones. In this work we present an NLG chatbot that processes natural language queries and provides insights through a combination of charts and text. We apply it to nutrition, a domain communication quality is critical. Through crowd-sourced evaluation we compare the informativeness of our chatbot against traditional, static diet-apps. We find that the conversational context significantly improved users understanding of dietary data in various tasks, and that users considered the chatbot as more useful and quick to use than traditional apps.

\section{Towards In-Context Non-Expert Evaluation of Reflection Generation for Counselling Conversations}

Reflection is an essential counselling strategy, where the therapist listens actively and responds with their own interpretation of the client’s words. Recent work leveraged pre-trained language models (PLMs) to approach reflection generation as a promising tool to aid counsellor training. However, those studies used limited dialogue context for modelling and simplistic error analysis for human evaluation. In this work, we take the first step towards addressing those limitations. First, we fine-tune PLMs on longer dialogue contexts for reflection generation. Then, we collect free-text error descriptions from non-experts about generated reflections, identify common patterns among them, and accordingly establish discrete error categories using thematic analysis. Based on this scheme, we plan for future work a mass non-expert error annotation phase for generated reflections followed by an expert-based validation phase, namely “whether a coherent and consistent response is a good reflection”.

\section{Data Augmentation for Reliability and Fairness in Counselling Quality Classification}

The mental health domain poses serious challenges to the validity of existing Natural Language Processing (NLP) approaches. Scarce and unbalanced data limits models’ reliability and fairness, therefore hampering real-world application. In this work, we address these challenges by using our recently released Anno-MI dataset, containing professionally annotated transcriptions in motivational interviewing (MI). To do so, we inspect the effects of data augmentation on classical machine (CML) and deep learning (DL) approaches for counselling quality classification. First, we adopt augmentation to balance the target label in order to improve the classifiers’ reliability. Next, we conduct the bias and fairness analysis by choosing the therapy topic as the sensitive variable. Finally, we implement a fairness-aware augmentation technique, showing how topic-wise bias can be mitigated by augmenting the target label with respect to the sensitive variable.Our work is the first step towards increa sing reliability and reducing the bias of classification models, as well as dealing with data scarcity and imbalance in mental health. 


\section{K-LM: Knowledge Augmenting in Language Models Within the Scholarly Domain}

The use of superior algorithms and complex architectures in language models have successfully imparted human-like abilities to machines for specific tasks. But two significant constraints, the available training data size and the understanding of domain-specific context, hamper the pre-trained language models from optimal and reliable performance. A potential solution to tackle these limitations is to equip the language models with domain knowledge. While the commonly adopted techniques use Knowledge Graphs Embeddings (KGEs) to inject domain knowledge, we provide a Knowledge Language Model (K-LM) to use the Resource Description Framework (RDF) triples directly, extracted from world knowledge bases. The proposed model works in conjunction with Generative Pretrained Transformer (GPT-2) and Bidirectional Encoder Representations from Transformers (BERT) and uses a well-defined pipeline to select, categorize, and filter the RDF triples. In addition, we introduce heuristic methods to inject domain-specific knowledge in K-LM, leveraging knowledge graphs (KGs). We tested our approaches on the classification task within the scholarly domain using two KGs, and our results show that our proposed language model has significantly outperformed the baselines and BERT for each KG. Our experimental findings also help us conclude the importance of relevance of KG used over the quantity of injected RDF triples. Also, each of our proposed methods for injecting the RDF triples has increased the overall model’s accuracy, demonstrating that K-LM is a potential choice for domain adaptation to solve knowledge-driven problems.

\section{Ensembling Classical Machine Learning and Deep Learning Approaches for Morbidity Identification From Clinical Notes}

The past decade has seen an explosion of the amount of digital information generated within the healthcare domain. Digital data exist in the form of images, video, speech, transcripts, electronic health records, clinical records, and free-text. Analysis and interpretation of healthcare data is a daunting task, and it demands a great deal of time, resources, and human effort. In this paper, we focus on the problem of co-morbidity recognition from patient's clinical records. To this aim, we employ both classical machine learning and deep learning approaches. We use word embeddings and bag-of-words representations, coupled with feature selection techniques. The goal of our work is to develop a classification system to identify whether a certain health condition occurs for a patient by studying his/her past clinical records. In more detail, we have used pre-trained word2vec, domain-trained, GloVe, fastText, and universal sentence encoder embeddings to tackle the classification of sixteen morbidity conditions within clinical records. We have compared the outcomes of classical machine learning and deep learning approaches with the employed feature representation methods and feature selection methods. We present a comprehensive discussion of the performances and behaviour of the employed classical machine learning and deep learning approaches. Finally, we have also used ensemble learning techniques over a large number of combinations of classifiers to improve the single model performance. For our experiments, we used the n2c2 natural language processing research dataset, released by Harvard Medical School. The dataset is in the form of clinical notes that contain patient discharge summaries. Given the unbalancedness of the data and their small size, the experimental results indicate the advantage of the ensemble learning technique with respect to single classifier models. In particular, the ensemble learning technique has slightly improved the performances of single classification models but has greatly reduced the variance of predictions stabilizing the accuracies (i.e., the lower standard deviation in comparison with single classifiers). In real-life scenarios, our work can be employed to identify with high accuracy morbidity conditions of patients by feeding our tool with their current clinical notes. Moreover, other domains where classification is a common problem might benefit from our approach as well.

\section{Towards Detecting Need for Empathetic Response in Motivational Interviewing}

Empathetic response from the therapist is key to the success of clinical psychotherapy, especially motivational interviewing. Previous work on computational modelling of empathy in motivational interviewing has focused on offline, session-level assessment of therapist empathy, where empathy captures all efforts that the therapistmakes to understand theclient's perspective and convey that understanding to the client. In this position paper, we propose a novel task of turn-level detection of client need for empathy. Concretely, we propose to leverage pre-trained language models and empathy-related general conversation corpora in a unique labeller-detector framework, where the labeller automatically annotates a motivational interviewing conversation corpus with empathy labels to train the detector that determines the need for therapist empathy. We also lay out our strategies of extending the detector with additional-input and multi-task setups to improve its detection and explainability.

\section{TF-IDF vs Word Embeddings for Morbidity Identification in Clinical Notes: An Initial Study}

Today, we are seeing an ever-increasing number of clinical notes that contain clinical results, images, and textual descriptions of patient's health state. All these data can be analyzed and employed to cater novel services that can help people and domain experts with their common healthcare tasks. However, many technologies such as Deep Learning and tools like Word Embeddings have started to be investigated only recently, and many challenges remain open when it comes to healthcare domain applications. To address these challenges, we propose the use of Deep Learning and Word Embeddings for identifying sixteen morbidity types within textual descriptions of clinical records. For this purpose, we have used a Deep Learning model based on Bidirectional Long-Short Term Memory (LSTM) layers which can exploit state-of-the-art vector representations of data such as Word Embeddings. We have employed pre-trained Word Embeddings namely GloVe and Word2Vec, and our own Word Embeddings trained on the target domain. Furthermore, we have compared the performances of the deep learning approaches against the traditional tf-idf using Support Vector Machine and Multilayer perceptron (our baselines). From the obtained results it seems that the latter outperforms the combination of Deep Learning approaches using any word embeddings. Our preliminary results indicate that there are specific features that make the dataset biased in favour of traditional machine learning approaches.

\section{Towards Low-Resource Real-Time Assessment of Empathy in Counselling}

Gauging therapist empathy in counselling is an important component of understanding counselling quality. While session-level empathy assessment based on machine learning has been investigated extensively, it relies on relatively large amounts of well-annotated dialogue data, and real-time evaluation has been overlooked in the past. In this paper, we focus on the task of low-resource utterance-level binary empathy assessment. We train deep learning models on heuristically constructed empathy vs. non-empathy contrast in general conversations, and apply the models directly to therapeutic dialogues, assuming correlation between empathy manifested in those two domains. We show that such training yields poor performance in general, probe its causes, and examine the actual effect of learning from empathy contrast in general conversation.

\section{Towards Automated Counselling Decision-Making: Remarks on Therapist Action Forecasting on the AnnoMI Dataset.}

Substantial progress has been made in recent years on natural language processing approaches to counselling conversation analysis. However, few studies have investigated therapist action forecasting, which aims to suggest dialogue actions that the therapist can take in the next turn, partly due to generally lim-ited access to counselling dialogue data resulting from privacy-related constraints. In this work, we leverage a recently released public dataset of therapy conversations and experiment with a range of natural language processing techniques to approach the task of therapist action forecasting with language models. We probe various factors that could impact model performance, including data augmentation, dialogue context length, incorporat-ing therapist/client utterance labels in the input, and contrasting high- and low-quality counselling dialogues. With our findings, we hope to provide insights on this task and inspire future efforts in counselling dialogue analysis.

\section{A Controllable Lifestyle Simulator for Use in Deep Reinforcement Learning Algorithms}

Deep learning, especially deep reinforcement learning (DRL), has become one of the most useful tools for solving sequential decision-making problems. This is particularly relevant to recommender systems and drug administration in healthcare. This approach has the main drawback of requiring a lot of training, usually several millions of examples before it can learn an interesting policy. Therefore, in healthcare, it is crucial for training the neural network to use reliable and realistic simulations of users. These simulations can be measurements of the user’s vital signals throughout the day or the occurrence of lifestyle events such as sleeping, eating, etc. In this paper, we present a novel and highly generalizable simulation system based on state machines associated with probabilistic transitions to simulate the user’s lifestyle. Thanks to its random nature, the proposed approach can generate infinite yet realistic data from the simulation. It can also be controlled based on the simulation constraints, which is an important requirement for DRL algorithms. We demonstrate its usefulness and relevance in two simple cases of user behavior simulation using different types of input data. We also show its application for a DRL scenario involving behavior change interventions.

\section{Neural Scoring of Logical Inferences from Data using Feedback}

Insights derived from wearable sensors in smartwatches or sleep trackers can help users in approaching their healthy lifestyle goals. These insights should indicate significant inferences from user behaviour and their generation should adapt automatically to the preferences and goals of the user. In this paper, we propose a neural network model that generates personalised lifestyle insights based on a model of their significance, and feedback from the user. Simulated analysis of our model shows its ability to assign high scores to a) insights with statistically significant behaviour patterns and b) topics related to simple or complex user preferences at any given time. We believe that the proposed neural networks model could be adapted for any application that needs user feedback to score logical inferences from data.

\section{Iterative Neural Scoring of Validated Insight Candidates}

Automatic generation of personalised behavioural insight messages is useful in many applications, for example, health selfmanagement services based on a wearable and an app. Insights should be statistically valid, but also interesting and actionable for the user of the service. In this paper, we propose a novel neural network approach for joint modeling of these elements of the relevancy, that is, statistical validity and user preference, using synthetic and real test data sets. We also demonstrate in an online learning scenario that the system can automatically adapt to the changing preferences of the user while preserving the statistical validity of the mined insights.

\section{Towards a Generalised Framework for Behaviour Insight Mining}

A behaviour insight is a statement t h a t explains the behaviour of a user's activity or a system's performance under certain conditions. Care must be taken to deliver insights in a way that is useful to the user. Mining for such insights and generating text to communicate about those is a complicated process and there is a need for standardisation to ensure it is done properly. In this work, we lay down the foundation towards a generalised behaviour insight mining framework based on our previous experiences in developing them and express our views on how it can be adopted in a wide range of applications such as Sleep, Marketing, Medical Image Diagnosis and clinical workflow management.

\section{Fully Autonomous Programming with Large Language Models}

Current approaches to program synthesis with Large Language Models (LLMs) exhibit a"near miss syndrome": they tend to generate programs that semantically resemble the correct answer (as measured by text similarity metrics or human evaluation), but achieve a low or even zero accuracy as measured by unit tests due to small imperfections, such as the wrong input or output format. This calls for an approach known as Synthesize, Execute, Debug (SED), whereby a draft of the solution is generated first, followed by a program repair phase addressing the failed tests. To effectively apply this approach to instruction-driven LLMs, one needs to determine which prompts perform best as instructions for LLMs, as well as strike a balance between repairing unsuccessful programs and replacing them with newly generated ones. We explore these trade-offs empirically, comparing replace-focused, repair-focused, and hybrid debug strategies, as well as different template-based and model-based prompt-generation techniques. We use OpenAI Codex as the LLM and Program Synthesis Benchmark 2 as a database of problem descriptions and tests for evaluation. The resulting framework outperforms both conventional usage of Codex without the repair phase and traditional genetic programming approaches.

\section{Neurogenetic programming framework for explainable reinforcement learning}

Automatic programming, the task of generating computer programs compliant with a specification without a human developer, is usually tackled either via genetic programming methods based on mutation and recombination of programs, or via neural language models. We propose a novel method that combines both approaches using a concept of a virtual neuro-genetic programmer, or scrum team. We demonstrate its ability to provide performant and explainable solutions for various OpenAI Gym tasks, as well as inject expert knowledge into the otherwise data-driven search for solutions.

\section{BF++: a language for general-purpose program synthesis}

Most state of the art decision systems based on Reinforcement Learning (RL) are data-driven black-box neural models, where it is often difficult to incorporate expert knowledge into the models or let experts review and validate the learned decision mechanisms. Knowledge-insertion and model review are important requirements in many applications involving human health and safety. One way to bridge the gap between data and knowledge driven systems is program synthesis: replacing a neural network that outputs decisions with one that generates decision-making code in some programming language. We propose a new programming language, BF++, designed specifically for neural program synthesis in a Partially Observable Markov Decision Process (POMDP) setting and generate programs for a number of standard OpenAI Gym benchmarks. 

\section{Towards Effective Patient Simulators}

In this paper we give an overview of the field of patient simulators and provide qualitative and quantitative comparison of different modeling and simulation approaches. Simulators can be used to train human caregivers but also to develop and optimize algorithms for clinical decision support applications and test and validate interventions. In this paper we introduce three novel patient simulators with different levels of representational accuracy: HeartPole, a simplistic transparent rule-based system, GraphSim, a graph-based model trained on intensive care data, and Auto-ALS—an adjusted version of an educational software package used for training junior healthcare professionals. We provide a qualitative and quantitative comparison of the previously existing as well as proposed simulators.

==> evals/diet.tex <==
% Diet coaching

As a starting point, we conducted extensive research to identify the limits of existing diet-coaching tools, both in terms of interaction and functionalities~\cite{10.1145/3450614.3463602}and emotional effect on the user~\cite{balloccu2020you}. The former is important as information quality impacts on dietary outcomes~\cite{van2008cognitive,savolainen2010dietary,michie2011behaviour}, while the latter is linked to research in nutrition repeatedly highlighting the relationship between emotions and diet behaviours~\cite{puddephatt2020eating,peng2018meta,riffer2019relationship}. 

Following this review, we proposed an initial architecture for a report generator~\cite{balloccu2020nlg}, consisting of considering users' personal goals and characteristics to generate personalised and engaging diet reports through rule-based NLG. We tested our approach in a 2-week trial~\cite{balloccu-reiter-2022-beyond} when we compared dietary outcomes of volunteers receiving and evaluating their report from our system, against a control group that used traditional diet apps. Notably, we implemented a number of text tailoring practices derived from Affective NLG~\cite{de1999affective,mahamood2011generating} and targeting the emotional load of dieting. To assess their effectiveness, we monitored the affective state of participants in both groups. From results, we observed an improved dietary outcome in presence of tailored communication but without statical
significance, hinting at the need for a longer experiment. Tailored communication also proved to significantly improve the emotional load of dieting compared to the control group. Participants showed to appreciate the system, with some requesting to use it after the trial.

Later on, we proposed an evolution of the framework consisting of a multimodal diet coaching chatbot~\cite{balloccu-reiter-2022-comparing} that combines visualisations and text to improve information understanding of dietary information. Thanks to this, our chatbot allowed users to quickly access both basic and advanced dietary insights. To assess whether this approach benefits informativeness, we tested it through human evaluation, with crowdworkers divided into three groups, using our chatbot or traditional diet apps to take a quiz. The quiz consisted of multiple-choice questions where the workers were asked to analyse a synthetic food diary and extract key facts from it. Our results showed that the chatbot group scored the highest on informativeness in almost every scenario. In multiple contexts, it significantly
outperformed traditional diet apps when informing users, which also expressed very positive feedback about it, and perceived it was the quickest and easiest tool to use.

==> referenc.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%
\biblstarthook{References may be \textit{cited} in the text either by number (preferred) or by author/year.\footnote{Make sure that all references from the list are cited in the text. Those not cited should be moved to a separate \textit{Further Reading} section or chapter.} The reference list should ideally be \textit{sorted} in alphabetical order -- even if reference numbers are used for the their citation in the text. If there are several works by the same author, the following order should be used: 
\begin{enumerate}
\item all works by the author alone, ordered chronologically by year of publication
\item all works by the author with a coauthor, ordered alphabetically by coauthor
\item all works by the author with several coauthors, ordered chronologically by year of publication.
\end{enumerate}
The \textit{styling} of references\footnote{Always use the standard abbreviation of a journal's name according to the ISSN \textit{List of Title Word Abbreviations}, see \url{http://www.issn.org/en/node/344}} depends on the subject of your book:
\begin{itemize}
\item The \textit{two} recommended styles for references in books on \textit{mathematical, physical, statistical and computer sciences} are depicted in ~\cite{science-contrib, science-online, science-mono, science-journal, science-DOI} and ~\cite{phys-online, phys-mono, phys-journal, phys-DOI, phys-contrib}.
\item Examples of the most commonly used reference style in books on \textit{Psychology, Social Sciences} are~\cite{psysoc-mono, psysoc-online,psysoc-journal, psysoc-contrib, psysoc-DOI}.
\item Examples for references in books on \textit{Humanities, Linguistics, Philosophy} are~\cite{humlinphil-journal, humlinphil-contrib, humlinphil-mono, humlinphil-online, humlinphil-DOI}.
\item Examples of the basic Springer style used in publications on a wide range of subjects such as \textit{Computer Science, Economics, Engineering, Geosciences, Life Sciences, Medicine, Biomedicine} are ~\cite{basic-contrib, basic-online, basic-journal, basic-DOI, basic-mono}. 
\end{itemize}
}

\begin{thebibliography}{99.}%
% and use \bibitem to create references.
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Contribution 
\bibitem{science-contrib} Broy, M.: Software engineering --- from auxiliary to key technologies. In: Broy, M., Dener, E. (eds.) Software Pioneers, pp. 10-13. Springer, Heidelberg (2002)
%
% Online Document
\bibitem{science-online} Dod, J.: Effective substances. In: The Dictionary of Substances and Their Effects. Royal Society of Chemistry (1999) Available via DIALOG. \\
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{science-mono} Geddes, K.O., Czapor, S.R., Labahn, G.: Algorithms for Computer Algebra. Kluwer, Boston (1992) 
%
% Journal article
\bibitem{science-journal} Hamburger, C.: Quasimonotonicity, regularity and duality for nonlinear systems of partial differential equations. Ann. Mat. Pura. Appl. \textbf{169}, 321--354 (1995)
%
% Journal article by DOI
\bibitem{science-DOI} Slifka, M.K., Whitton, J.L.: Clinical implications of dysregulated cytokine production. J. Mol. Med. (2000) doi: 10.1007/s001090000086 
%
\bigskip

% Use the following (APS) syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Online Document
\bibitem{phys-online} J. Dod, in \textit{The Dictionary of Substances and Their Effects}, Royal Society of Chemistry. (Available via DIALOG, 1999), 
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{phys-mono} H. Ibach, H. L\"uth, \textit{Solid-State Physics}, 2nd edn. (Springer, New York, 1996), pp. 45-56 
%
% Journal article
\bibitem{phys-journal} S. Preuss, A. Demchuk Jr., M. Stuke, Appl. Phys. A \textbf{61}
%
% Journal article by DOI
\bibitem{phys-DOI} M.K. Slifka, J.L. Whitton, J. Mol. Med., doi: 10.1007/s001090000086
%
% Contribution 
\bibitem{phys-contrib} S.E. Smith, in \textit{Neuromuscular Junction}, ed. by E. Zaimis. Handbook of Experimental Pharmacology, vol 42 (Springer, Heidelberg, 1976), p. 593
%
\bigskip
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Psychology, Social Sciences"
%
%
% Monograph
\bibitem{psysoc-mono} Calfee, R.~C., \& Valencia, R.~R. (1991). \textit{APA guide to preparing manuscripts for journal publication.} Washington, DC: American Psychological Association.
%
% Online Document
\bibitem{psysoc-online} Dod, J. (1999). Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
\url{http://www.rsc.org/dose/Effective substances.} Cited 15 Jan 1999.
%
% Journal article
\bibitem{psysoc-journal} Harris, M., Karper, E., Stacks, G., Hoffman, D., DeNiro, R., Cruz, P., et al. (2001). Writing labs and the Hollywood connection. \textit{J Film} Writing, 44(3), 213--245.
%
% Contribution 
\bibitem{psysoc-contrib} O'Neil, J.~M., \& Egan, J. (1992). Men's and women's gender role journeys: Metaphor for healing, transition, and transformation. In B.~R. Wainrig (Ed.), \textit{Gender issues across the life cycle} (pp. 107--123). New York: Springer.
%
% Journal article by DOI
\bibitem{psysoc-DOI}Kreger, M., Brindis, C.D., Manuel, D.M., Sassoubre, L. (2007). Lessons learned in systems change initiatives: benchmarks and indicators. \textit{American Journal of Community Psychology}, doi: 10.1007/s10464-007-9108-14.
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Humanities, Linguistics, Philosophy"
%
\bigskip
%
% Journal article
\bibitem{humlinphil-journal} Alber John, Daniel C. O'Connell, and Sabine Kowal. 2002. Personal perspective in TV interviews. \textit{Pragmatics} 12:257--271
%
% Contribution 
\bibitem{humlinphil-contrib} Cameron, Deborah. 1997. Theoretical debates in feminist linguistics: Questions of sex and gender. In \textit{Gender and discourse}, ed. Ruth Wodak, 99--119. London: Sage Publications.
%
% Monograph
\bibitem{humlinphil-mono} Cameron, Deborah. 1985. \textit{Feminism and linguistic theory.} New York: St. Martin's Press.
%
% Online Document
\bibitem{humlinphil-online} Dod, Jake. 1999. Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999
%
% Journal article by DOI
\bibitem{humlinphil-DOI} Suleiman, Camelia, Daniel C. O?Connell, and Sabine Kowal. 2002. `If you and I, if we, in this later day, lose that sacred fire...?': Perspective in political interviews. \textit{Journal of Psycholinguistic Research}. doi: 10.1023/A:1015592129296.
%
%
%
\bigskip
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Computer Science, Economics, Engineering, Geosciences, Life Sciences"
%
%
% Contribution 
\bibitem{basic-contrib} Brown B, Aaron M (2001) The politics of nature. In: Smith J (ed) The rise of modern genomics, 3rd edn. Wiley, New York 
%
% Online Document
\bibitem{basic-online} Dod J (1999) Effective Substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Journal article by DOI
\bibitem{basic-DOI} Slifka MK, Whitton JL (2000) Clinical implications of dysregulated cytokine production. J Mol Med, doi: 10.1007/s001090000086
%
% Journal article
\bibitem{basic-journal} Smith J, Jones M Jr, Houghton L et al (1999) Future of health insurance. N Engl J Med 965:325--329
%
% Monograph
\bibitem{basic-mono} South J, Blass B (2001) The future of modern genomics. Blackwell, London 
%

\end{thebibliography}

